A Reusable Component for Communication and Data Synchronization in Mobile Distributed Interactive Applications

In Distributed Interactive Applications (DIA) such as multiplayer games, where many participants are involved in a same game session and communicate through a network, they may have an inconsistent view of the virtual world because of the communication delays across the network. This issue becomes even more challenging when communicating through a cellular network while executing the DIA client on a mobile terminal. Consistency maintenance algorithms may be used to obtain a uniform view of the virtual world. These algorithms are very complex and hard to program and therefore, the implementation and the future evolution of the application logic code become difficult. To solve this problem, we propose an approach where the consistency concerns are handled separately by a distributed component called a Synchronization Medium, which is responsible for the communication management as well as the consistency maintenance. We present the detailed architecture of the Synchronization Medium and the generic interfaces it offers to DIAs. We evaluate our approach both qualitatively and quantitatively. We first demonstrate that the Synchronization Medium is a reusable component through the development of two game applications, a car racing game and a space war game. A performance evaluation then shows that the overhead introduced by the Synchronization Medium remains acceptable.

==> eptcsdata.tex <==
\providecommand{\firstpage}{86}
\providecommand{\publicationstatus}{C\'amara, Canal, and Sala\"un (Eds.) \\
Component and Service Interoperability (WCSI10)\\
EPTCS 37, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.37.7}{10.4204/EPTCS.37.7}}

